SOCIA-EVO: Automated Simulator Construction via Dual-Anchored Bi-Level Optimization

Automated simulator construction requires distributional fidelity, distinguishing it from generic code generation. We identify two failure modes in long-horizon LLM agents: contextual drift and optimization instability arising from conflating structural and parametric errors. We propose SOCIA-EVO, a dual-anchored evolutionary framework. SOCIA-EVO introduces: (1) a static blueprint to enforce empirical constraints; (2) a bi-level optimization to decouple structural refinement from parameter calibration; and (3) a self-curating Strategy Playbook that manages remedial hypotheses via Bayesian-weighted retrieval. By falsifying ineffective strategies through execution feedback, SOCIA-EVO achieves robust convergence, generating simulators that are statistically consistent with observational data. The code and data of SOCIA-EVO are available here: https://github.com/cruiseresearchgroup/SOCIA/tree/evo.

==> latex/chapter/1_intro_backup.tex <==
%
The automated construction of simulators from observational data---often termed \emph{data-driven simulation}---is a cornerstone for understanding complex systems, ranging from epidemiological modeling to user behavior modeling. 
Unlike generic software engineering, where success is typically defined by functional correctness (i.e., ``does the code execute without errors?''), simulator construction is fundamentally a \emph{scientific modeling} task. 
The generated program must not only be syntactically valid, but also exhibit \emph{distributional fidelity}: it should faithfully reproduce the statistical properties, causal mechanisms, and emergent behaviors observed in the ground-truth data. 
While large language models (LLMs) have demonstrated remarkable proficiency in translating natural language into code, applying them to this high-stakes, multi-objective optimization setting remains an open challenge. 
In particular, moving from a static dataset to a dynamic, executable simulation requires an agent to bridge a substantial semantic gap, while maintaining rigorous consistency between the generated logic and empirical constraints.

We identify two critical failure modes that arise when standard LLM-based agents are applied to this task over long horizons. The first is \emph{contextual drift}. 
As simulator complexity increases---with intricate state transitions, heterogeneous entities, and rich interaction dynamics---the strict constraints established during the initial data analysis gradually lose salience in the model's attention. Agents may begin to hallucinate governing rules or disregard data schemas that were explicitly specified at the outset. 
In the absence of a persistent, authoritative anchor, the agent's objective can implicitly shift from \emph{data fidelity} to mere \emph{code completion}, yielding simulators that are syntactically plausible yet physically or statistically invalid.

Second, and more critically, agents often exhibit \emph{optimization instability} throughout the calibration process. We attribute this failure to two compounding factors. The first is the \emph{conflation of structure and parameters}. Simulator calibration is inherently a multi-objective optimization problem, yet LLM-based agents frequently fail to disentangle \emph{structural flaws} (e.g., incorrect transition logic or missing mechanisms) from \emph{parametric misalignment} (e.g., suboptimal constants or rates). As a result, an agent may wastefully rewrite otherwise-correct logic when a simple parameter adjustment would suffice---behaving like a ``whack-a-mole'' player who changes the rules of the game instead of improving their aim. 

This reasoning deficit is further exacerbated by a memory failure analogous to \emph{catastrophic forgetting}. As the context window advances, the agent loses access to \emph{negative knowledge}---failed attempts, rejected hypotheses, and constraints learned through trial and error in earlier iterations. Without a persistent memory to track these oscillatory trajectories, the agent is prone to revisiting ineffective strategies, thereby impeding convergence toward a high-fidelity model.

% While recent advances have addressed individual aspects of this problem, they do not yet provide a holistic solution for data-driven simulator construction.

% \emph{(i) General-purpose context evolution is insufficient.}
% Methods such as Iterative Reflexion, Dynamic Cheatsheets, and agentic context engineering (ACE) aim to summarize interaction history to preserve logical coherence over long horizons. However, these techniques are largely \emph{metric-agnostic}: they treat code generation primarily as a semantic completion problem rather than a scientific modeling problem. As a result, they lack mechanisms to ground context updates in quantitative simulation feedback (e.g., distributional distances or calibration objectives). The resulting ``cheatsheets'' often retain generic coding advice but fail to encode \emph{causal failure signatures} specific to calibration. Without an explicit \emph{blueprint} that persistently anchors empirical constraints, these approaches remain vulnerable to the contextual drift described above.

% \emph{(ii) Existing LLM-based simulation frameworks sidestep environment construction.}
% Several LLM-driven simulation systems focus on generating realistic agent behaviors \emph{within} a predefined environment. They typically assume the simulator's rules, physics, and topology are given or fixed, and therefore do not confront the core challenge studied here: \emph{constructing} the simulator itself from observational data such that its outputs match ground-truth statistics.

% \emph{(iii) Generative simulation lacks long-horizon evolutionary memory.}
% Approaches that combine LLMs with gradient-free calibration can improve fidelity, but they often behave as short-horizon optimizers. In particular, they rarely maintain persistent, structured memory that retains \emph{negative knowledge} across dozens of iterations---failed hypotheses, rejected structural variants, and non-improving parameter regions. Consequently, under the ``whack-a-mole'' trade-offs inherent to multi-objective calibration, such systems are prone to optimization instability: they may revisit ineffective structural changes or oscillate among local optima without accumulating durable learning from historical trajectories.

Existing approaches fall short of a holistic solution for this specific problem. General context evolution methods, such as Iterative Reflexion, Dynamic Cheatsheets, and generic ACE, are predominantly metric-agnostic; they optimize for semantic coherence rather than quantitative calibration, lacking the feedback loops to ground code changes in distributional metrics . Conversely, domain-specific works like YuLan-OneSim focus on generating agent behaviors within pre-defined environments, neglecting the fundamental challenge of constructing the simulator logic itself from observational data. Even generative frameworks like G-Sim, which incorporate calibration, lack a persistent evolutionary memory (i.e., a structured Playbook) to track "negative knowledge" across long horizons , leaving them vulnerable to the optimization instability and redundant exploration described above .

% To address these gaps, we introduce \textsc{SOCIA-ACE}, an agentic context engineering framework tailored to automated simulator construction. \textsc{SOCIA-ACE} reconceptualizes code generation as a \emph{dual-anchored evolutionary} process. To mitigate contextual drift, we introduce a \emph{Blueprint}: a static, authoritative specification distilled from rigorous data analysis. The Blueprint serves as a set of \emph{ground-truth requirements}, anchoring the agent's generative trajectory to the dataset's immutable statistical constraints.

% Crucially, \textsc{SOCIA-ACE} adopts a \emph{bi-level optimization} strategy that decouples structural reasoning from parameter search. In the outer loop, the agent iteratively refines the discrete simulator architecture under the Blueprint's constraints. In the inner loop, the system automatically synthesizes a numerical calibrator to optimize continuous parameters. This separation ensures that the feedback presented to the agent reflects the intrinsic limitations of the current \emph{model structure}, rather than confounding noise from untuned parameters.

% To prevent the recurrence of previously resolved bugs and mitigate ``catastrophic forgetting,'' we propose a \emph{Strategy Playbook} mechanism. Rather than storing unstructured textual traces, the Playbook maintains \emph{structured diagnostic records} grounded in empirical evidence by enforcing explicit links between code deficiencies and specific metric failures. The Playbook functions as an \emph{evolutionary memory}, managing strategies via a formal state machine (e.g., \textsc{Open}, \textsc{Resolved}, \textsc{Persist}). In particular, it explicitly identifies and penalizes strategies that consistently degrade metrics (the \textsc{Persist} state), thereby ``freezing'' hard-won lessons from failure.

% To further overcome the finite context window, we cast context management as a \emph{resource allocation} problem. We introduce a knapsack-based selection algorithm that dynamically curates the most valuable strategies---weighted by Bayesian reliability estimates and urgency---so that the agent's working context is consistently populated with the most critical \emph{negative knowledge}, reducing regression across long-horizon iterations.

To address these gaps, we introduce \textsc{SOCIA-ACE}, which reconceptualizes automated simulator construction as a \emph{dual-anchored evolutionary} process. 
First, to mitigate contextual drift, we establish a \emph{Blueprint}---a static, authoritative specification distilled from data analysis---that anchors the agent to immutable statistical constraints. 
Crucially, we implement a \emph{bi-level optimization} strategy that decouples structural reasoning from parameter search. By delegating continuous parameter tuning to an inner numerical loop while allowing the agent to refine the discrete simulator architecture in the outer loop, the resulting feedback more accurately reflects intrinsic structural limitations, rather than being confounded by noise from untuned parameters.

Second, to reduce ``catastrophic forgetting,'' we propose a \emph{Strategy Playbook} that stores structured diagnostic records instead of unstructured textual traces. Grounded in empirical evidence, the Playbook manages strategies through a metric-driven state machine, explicitly penalizing strategies that reliably degrade performance (the \textsc{Persist} state), thereby ``freezing'' hard-won lessons from failure. 
Finally, treating the finite context window as a resource allocation constraint, we employ a knapsack-based selection algorithm to curate what enters the agent's working context. Weighted by Bayesian reliability estimates, this algorithm dynamically prioritizes the most critical \emph{negative knowledge}, helping prevent regression across long-horizon iterations.


Our contributions are threefold:
\begin{itemize}
    \item We formalize \emph{Automated Simulator Construction} as a dual-anchored agentic task, distinguishing it from generic code generation by its emphasis on \emph{distributional fidelity} and its susceptibility to \emph{optimization instability} during calibration.
    \item We propose \textsc{SOCIA-ACE}, a framework that introduces (i) a bi-level optimization architecture to decouple parameter calibration from structural refinement, and (ii) a \emph{Blueprint} mechanism to enforce consistency with empirical data constraints.
    \item We design a \emph{metric-driven Playbook} that maintains structured, evidence-grounded repair strategies using a state machine and a knapsack-based selection algorithm, mitigating catastrophic forgetting by preserving and prioritizing \emph{negative knowledge}.
\end{itemize}


















==> latex/chapter/1_intro_obsolete.tex <==
%
The automated construction of simulators from observational data—\emph{data-driven simulation}—is a cornerstone for understanding complex systems. 
Unlike generic software engineering where functional correctness suffices, simulator construction is fundamentally a \emph{scientific modeling} task requiring \emph{distributional fidelity}. 
The generated program must reproduce the statistical regularities, causal mechanisms, and emergent behaviors of the ground truth. 
While Large Language Models (LLMs) demonstrate strong capabilities in translating natural language into code, applying them to this domain remains challenging. 
Moving from a static dataset to a dynamic, executable simulation requires bridging a substantial semantic gap while maintaining rigorous consistency with empirical constraints.


% \vspace{0.25em}
% \noindent
% We identify two critical failure modes that arise when standard LLM-based agents are applied to automated simulator construction over long horizons. 
% The first is \emph{contextual drift}. 
% As simulator complexity increases—with intricate state transitions, heterogeneous entities, and rich interaction dynamics—constraints established during the initial data analysis gradually lose salience in the model's attention. 
% Agents may begin to hallucinate governing rules, violate data schemas, or introduce mechanisms that were never supported by evidence. 
% Without a persistent and authoritative anchor, the agent's implicit objective can shift from \emph{data fidelity} to mere \emph{code completion}, yielding simulators that are syntactically plausible yet physically or statistically invalid.


% \vspace{0.25em}
% \noindent
% The second, and more critical, failure mode is \emph{optimization instability} during calibration. 
% First, agents frequently \emph{conflate structure and parameters}, failing to distinguish structural flaws (e.g., incorrect transition logic) from parametric misalignment (e.g., suboptimal rates). 
% Consequently, an agent may rewrite otherwise-correct logic when simple tuning would suffice, leading to oscillatory modifications analogous to a `whack-a-mole' game. 
% Second, this reasoning challenge is exacerbated by the lack of a mechanism to verify and retain \emph{corrective insights}. 
% As the context window advances, the agent loses access to previous diagnostic feedbacks—failed attempts and rejected hypotheses from earlier iterations. 
% Lacking a persistent memory of what \emph{not} to do, the agent repeatedly rediscovers mistakes, impeding convergence toward a high-fidelity model.

\vspace{0.25em}
\noindent
We identify two critical failure modes in long-horizon simulator construction. The first is \emph{contextual drift}. As simulator complexity increases, agents tend to lose focus on initial constraints, hallucinating governing rules or violating data schemas. Without a persistent anchor, the objective implicitly shifts from \emph{data fidelity} to mere \emph{code completion}, yielding syntactically plausible but statistically invalid simulators.
The second is \emph{optimization instability}. Agents frequently conflate structural flaws with parametric misalignment, leading to oscillatory, ``whack-a-mole'' logic rewrites when simple tuning would suffice. This instability is exacerbated by the lack of a persistent memory for \emph{corrective insights}. As the context window moves, agents lose access to prior diagnostic feedback, repeatedly rediscovering previously falsified hypotheses and impeding convergence.

\vspace{0.25em}
\noindent
Recent work addresses fragments of long-horizon LLM agents, but does not yet offer a holistic solution for \emph{data-driven simulator construction}.
General-purpose context evolution methods—including Reflexion~\cite{shinn2023reflexion}, TextGrad~\cite{DBLP:journals/corr/abs-2406-07496}, and ACE~\cite{zhang2025agentic}—are largely \emph{metric-agnostic}, improving semantic coherence without grounding revisions in quantitative simulation feedback (e.g., distributional distances), and thus remain vulnerable to drift.
Conversely, domain-specific LLM simulation frameworks such as YuLan-OneSim~\cite{wang2025yulan} focus on generating agent behaviors \emph{within} pre-defined environments, implicitly assuming simulator rules are fixed rather than \emph{constructed}.
Finally, even calibration-aware generative methods such as G-Sim~\cite{DBLP:journals/corr/abs-2506-09272} typically operate as short-horizon optimizers and lack persistent, structured memory to retain and prioritize \emph{negative knowledge} across many iterations, leading to redundant exploration and optimization instability.
Critically, existing methods lack a structured mechanism to distinctively manage \emph{foundational rules} versus \emph{corrective adaptations}, leading to redundant exploration.

\begin{figure*}[t]
\centering
\includegraphics[width=1.0\textwidth]{latex/figure/socia-ace-framework.png} 
\caption{The \socia framework. The process is dual-anchored by a static \textit{Blueprint} ($\mathcal{B}$) and a dynamic \textit{Strategy Playbook} ($\mathcal{K}$). A bi-level optimization decouples structural refinement (Outer Loop) from parameter calibration (Inner Loop), leveraging metric-driven feedback to evolve strategies and prevent optimization instability.}
\label{fig:framework}
% \vspace{-1em}
\end{figure*}

\vspace{0.25em}
\noindent
To bridge this gap, we propose \textbf{\socia}, a framework that reconceptualizes automated simulator construction as an \emph{evolutionary feedback control system} driven by orthogonal knowledge streams. 
Unlike monolithic generation approaches, \socia synthesizes two distinct forces: a static, positive baseline for construction, and a dynamic, corrective gradient for calibration.
Formally, the code generation process at iteration $t+1$ is modeled as a vector synthesis:
\begin{equation}
\label{eq:framework_logic}
\begin{aligned}
Code_{t+1} 
  &= \underbrace{\text{Blueprint}(V_{base})}_{\text{Expert-aligned structure}} \\
  &\quad+ \underbrace{\sum \text{Selected remedial strategies}(\Delta V)}_{\text{Data-driven correction}}
\end{aligned}
\end{equation}

\noindent
This formulation underpins our three-stage methodology:
\textbf{First}, we establish the Hybrid Blueprint ($V_{base}$), a static foundation merging LLM priors with expert-verified constraints. 
This anchors the agent to the "lower bound" of structural correctness, preventing contextual drift.
\textbf{Second}, to provide the optimization gradient ($\Delta V$), we introduce a \emph{Strategy Playbook} that stores Remedial Strategies—dynamic insights derived from diagnostic feedback.
\textbf{Third}, we implement a \emph{Hypothesis Verification Loop} to solve optimization instability. 
Recognizing that LLM-generated strategies are merely hypotheses, the system employs a knapsack-based selection algorithm to prioritize empirically successful strategies while strictly "freezing" (discarding) falsified strategies that fail to improve simulation fidelity. 
This ensures \emph{self-sanitization}, allowing the agent to continuously refine its logic by learning from both positive verification and negative falsification.


\vspace{0.25em}
\noindent
\textbf{Contributions.}
Our contributions are threefold: 
\textbf{(1) Framework:} We formalize Simulator Construction as a \emph{dual-anchored evolutionary task}, distinguishing it from generic code generation by modeling it as the synergy of two orthogonal streams: expert-aligned construction and data-driven calibration. 
\textbf{(2) Mechanism:} We propose \socia, which introduces a \emph{Hybrid Blueprint} to enforce consistency and a \emph{Metric-Driven Playbook} equipped with a \emph{falsification-based freezing mechanism}, ensuring that only effective remedial strategies drive the code evolution. 
\textbf{(3) Performance:} We demonstrate that this synergistic approach significantly outperforms standard agentic workflows in achieving distributional fidelity and convergence stability across complex simulation scenarios.

==> latex/chapter/2_appro_obsolete.tex <==
\subsection{Problem Formulation \& Overview}
\label{sec:problem_formulation}

We formalize Automated Simulator Construction as a search problem within the space of executable programs. 
As shown in Figure~\ref{fig:framework}, given an observational dataset $\mathcal{D}_{obs}$ and a task specification $\mathcal{I}$, the goal is to synthesize a simulator $S$ parameterized by discrete code structure $P$ and continuous parameters $\theta$. 
The optimization objective is to minimize the distributional distance between the simulated data $\mathcal{D}_{sim} \sim S(P, \theta)$ and $\mathcal{D}_{obs}$:
\begin{equation}
    (P^*, \theta^*) = \mathop{\arg\min}_{P, \theta} \text{Dist}\left( S(P, \theta), \mathcal{D}_{obs} \right)
\end{equation}
To solve this problem efficiently, \socia employs a closed-loop iterative workflow involving five specialized agents. 
As outlined in Algorithm~\ref{alg:socia_ace}, the process begins with the \textbf{Data Analysis Agent}, which synthesizes a static \textit{Blueprint} ($\mathcal{B}$) to anchor the search space. 
The system then enters an evolutionary loop: 
(1) The \textbf{Code Generation Agent} synthesizes simulator code $P_t$ and a parameter calibrator $C_t$ based on $\mathcal{B}$ and the current \textit{Playbook} strategies $\mathcal{K}$; 
(2) The \textbf{Simulation Execution Agent} executes $C_t$ to optimize $\theta$ (inner loop) and runs the simulation to obtain metrics $\mathcal{M}_t$; 
(3) The \textbf{Feedback Generation Agent} diagnoses discrepancies between $\mathcal{M}_t$ and $\mathcal{B}$; 
(4) The \textbf{Playbook Manager} updates the remedial strategy repository $\mathcal{K}$; 
(5) The \textbf{Iteration Control Agent} evaluates convergence to decide whether to terminate.

\begin{algorithm}[t]
\caption{\socia Framework Flow}
\label{alg:socia_ace}
\begin{algorithmic}[1]
\Require Observational Data $\mathcal{D}_{obs}$, User Intent $\mathcal{I}$
\Ensure Optimized Simulator $S(P^*, \theta^*)$
\State $\mathcal{B} \gets \text{DataAnalysisAgent}(\mathcal{D}_{obs}, \mathcal{I})$ \Comment{Generate Blueprint (Static Anchor)}
\State $\mathcal{K} \gets \emptyset$, $P_0 \gets \text{InitCode}(\mathcal{B})$ \Comment{Initialize Playbook \& Code}
\State $t \gets 0$
\While{not \text{Converged}}
    \State \textcolor{blue}{\textit{// Step 1: Context Engineering via Playbook}}
    \State $\mathcal{S}_{sel} \gets \text{KnapsackSelect}(\mathcal{K}, \text{Budget})$ \Comment{Select strategies from Playbook}
    
    \State \textcolor{blue}{\textit{// Step 2: Outer Loop (Structure Refinement)}}
    \State $P_t, C_t \gets \text{CodeGenAgent}(\mathcal{B}, \mathcal{S}_{sel}, P_{t-1})$
    
    \State \textcolor{blue}{\textit{// Step 3: Inner Loop (Parameter Calibration) \& Execution}}
    \State $\theta_t^* \gets \text{CalibratorExec}(C_t, \mathcal{D}_{obs})$ \Comment{Optimize continuous params}
    \State $\mathcal{M}_t \gets \text{SimExecAgent}(P_t, \theta_t^*)$ \Comment{Get metrics (Distribution fidelity)}
    
    \State \textcolor{blue}{\textit{// Step 4: Metric-Driven Feedback}}
    \State $F_t \gets \text{FeedbackGenAgent}(\mathcal{M}_t, \mathcal{B}, P_t)$
    
    \State \textcolor{blue}{\textit{// Step 5: Strategy Evolution}}
    \State $\mathcal{K} \gets \text{UpdatePlaybook}(\mathcal{K}, F_t)$ \Comment{Merge \& State Update (Open/Resolved)}
    
    \If{$\text{IterationControlAgent}(\mathcal{M}_t)$ is \textsc{Stop}}
        \State \textbf{break}
    \EndIf
    \State $t \gets t + 1$
\EndWhile
\State \textbf{return} $S(P_t, \theta_t^*)$
\end{algorithmic}
\end{algorithm}


\subsection{The Static Anchor: Blueprint-Driven Bi-Level Optimization}
\label{sec:blueprint_bilevel}

To mitigate context drift and the conflation of structural and parametric errors, \socia establishes a static reference frame and separates the optimization search space.

\subsubsection{The Blueprint as Ground Truth}
The \textbf{Blueprint} ($\mathcal{B}$) serves as the authoritative specification for the simulator. Unlike dynamic prompts or file summaries that evolve and potentially decay over long horizons, $\mathcal{B}$ functions as a set of \textbf{immutable constraints} anchoring the generative process to the ground truth. 
Structurally, $\mathcal{B}$ rigorously defines the simulation topology, agent schemas (roles, states, attributes), exogenous signals, and crucial evaluation metrics aligned with $\mathcal{D}_{obs}$. 
To ensure domain alignment, we incorporate a human-in-the-loop verification step where experts review and iteratively refine the initial $\mathcal{B}$ via natural language feedback before the optimization loop begins . 
This preemptive intervention prevents the search from initializing in an invalid subspace, ensuring that all subsequent iterations adhere to a valid trajectory verified by domain knowledge.

\subsubsection{Bi-Level Optimization Strategy}
A core challenge in simulator construction is that structural flaws (e.g., missing feedback loops) and parametric misalignment (e.g., incorrect coefficients) often manifest as similar metric deviations. 
LLMs, while adept at discrete logical reasoning, struggle with high-dimensional continuous parameter search. 
To address this, we formulate the code generation process as a \textbf{bi-level optimization problem}, decoupling the discrete search for program structure $P$ from the continuous optimization of parameters $\theta$.

\paragraph{Outer Loop: Structural Refinement.}
The outer loop performs a discrete search over the space of valid programs. At iteration $t$, the Code Generation Agent acts as a policy $\pi_{code}$, synthesizing the simulator structure $P_t$ and a corresponding parameter calibrator $C_t$:
\begin{equation}
    (P_t, C_t) \leftarrow \pi_{code}(P_{t-1}, \mathcal{B}, \mathcal{K})
\end{equation}
where $\mathcal{B}$ ensures schema compliance and $\mathcal{K}$ (Playbook) provides evolutionary strategies. Crucially, the agent does not guess $\theta$; instead, it synthesizes the \textit{optimization procedure} ($C_t$) required to find them.

\paragraph{Inner Loop: Parameter Calibration.}
The inner loop executes the synthesized calibrator $C_t$, which employs a numerical optimizer (e.g., Tree-structured Parzen Estimator) to solve for the optimal parameters $\theta_t^*$ under the fixed structure $P_t$:
\begin{equation}
    \theta_t^* = \mathop{\arg\min}_{\theta \in \Theta} \mathcal{L}\left( \text{Sim}(P_t, \theta), \mathcal{D}_{obs} \right)
\end{equation}
where $\mathcal{L}$ is the loss function derived from the metrics defined in $\mathcal{B}$.

This separation ensures that the performance metrics $\mathcal{M}_t = \mathcal{L}(P_t, \theta_t^*)$ observed by the Feedback Agent represent the \textit{intrinsic capacity} of the structure $P_t$ . 
By evaluating $P_t$ at its parametric optimum, the system effectively filters out noise from untuned parameters, allowing the Feedback Agent to accurately attribute remaining deficits to structural logic rather than calibration errors.

\paragraph{Iteration Control Policy.}
Unlike fixed-step optimization, our agent dynamically terminates the outer loop based on a prioritized logic. It enforces hard guardrails to block stopping if critical diagnostic issues persist or performance regresses ($>3\%$). Conversely, it triggers soft termination to save compute when an optimization plateau is detected (insignificant gains over 2 iterations) or the system reaches a clean state. This ensures the simulator is both statistically valid and cost-effective.

\subsection{The Dynamic Anchor: Metric-Driven Strategy Playbook}
\label{sec:playbook}
To counteract optimization instability and the loss of validated remediation history over long horizons, \socia employs a dynamic evolutionary memory. Unlike passive logs, the \textbf{Strategy Playbook} ($\mathcal{K}$) maintains a repository of \emph{Remedial Strategies}---actionable repair hypotheses grounded in metric-driven diagnosis---and manages their lifecycle through a formal state machine. Importantly, these strategies are not treated as ``truth'': LLM-generated remediation suggestions can be wrong due to misattribution or spurious correlations. Therefore, the Playbook is designed to \emph{validate strategies by execution} and \emph{self-purify} by downgrading or pruning strategies that consistently fail to improve metrics.

\subsubsection{Structured Strategy Representation}
We formally define the Playbook as a set of strategies $\mathcal{K} = \{S_1, S_2, \dots, S_N\}$. Each strategy $S_i$ is not a mere textual trace but a structured tuple $S_i = \langle R_i, M_i, \Sigma_i \rangle$:

\begin{itemize}
    \item \textbf{Reflection ($R_i$)}: Encapsulates the diagnostic content, including the identified root cause, the proposed corrective approach, and critically, the \textit{metric links} set $\Lambda_i \subset \mathcal{M}$. The set $\Lambda_i$ explicitly binds the structural defect to specific simulation metrics (defined in the Blueprint $\mathcal{B}$), enabling evidence-based retrieval.
    \item \textbf{Meta-info ($M_i$)}: Maintains evolutionary statistics to estimate reliability. It is a triplet $(u_i, s_i, f_i)$ representing the \textit{usage count} (times selected), \textit{success attribution} (times resolved), and \textit{failure attribution} (times causing regression), respectively.
    \item \textbf{Status ($\Sigma_i$)}: A label from the finite state set $\mathcal{Q}$ indicating the strategy's current lifecycle phase.
\end{itemize}

\subsubsection{The Evolutionary State Machine}
The evolution of strategies is modeled as a transition system over the state space $\mathcal{Q} = \{ \textsc{Open}, \textsc{Queued}, \textsc{InProgress}, \textsc{Resolved} \}$. 
Transitions are triggered by discrete events $E$ derived from both the context engineering phase and the feedback evaluation phase.
Table~\ref{tab:state_transition} details the complete transition logic.

We categorize these transitions into two phases:

\paragraph{1. Selection \& Lifecycle Events.}
These events dictate which strategies enter the agent's context window:
\begin{itemize}
    \item \textbf{$E_{new}$ (Initialization)}: Triggered when the Feedback Agent identifies a defect $S_{new}$ that has no semantic match in $\mathcal{K}$ (i.e., $\max Sim(S_{new}, S_{hist}) < \delta_{thresh}$). A new strategy is initialized in \textsc{Open} with counters $(0,0,0)$.
    \item \textbf{$E_{merge}$ (Recurrence)}: Triggered when a new defect matches an existing strategy $S_{hist}$ (detailed in Sec.~\ref{ssec:playbook_merge}). The strategy resets to \textsc{Open} to be re-addressed, while preserving its historical counters to maintain reliability estimates.
    \item \textbf{$E_{selected}$ / $not\_selected$ (Scheduling)}: Driven by the knapsack optimization (Sec.~\ref{ssec:knapsack}). If strategy $S_i$ is selected for the prompt ($x_i=1$), $E_{selected}$ fires, transitioning it to \textsc{InProgress} and incrementing usage ($u_i \leftarrow u_i + 1$). Strategies not selected due to budget constraints trigger $not\_selected$, moving to (or remaining in) \textsc{Queued} to reflect backlog aging.
\end{itemize}

\paragraph{2. Metric-Driven Feedback Events.}
Upon execution of the bi-level optimization, the resulting metric changes ($\Delta \mathcal{M}$) trigger evaluation events:
\begin{itemize}
    \item \textbf{$E_{resolved}$ (Validation Success)}: Triggered when linked metrics improve significantly ($\Delta \mathcal{M} > \tau$). The strategy transitions to \textsc{Resolved}, and the success counter is incremented ($s_i \leftarrow s_i + 1$). This provides \emph{empirical validation} that the remediation hypothesis is beneficial in practice.
    \item \textbf{$E_{persist}$ (Falsification / Harm Evidence)}: Triggered when linked metrics degrade significantly ($\Delta \mathcal{M} < -\tau$). This suggests the selected remediation hypothesis was ineffective or harmful. The strategy is returned to the \textsc{Open} pool for reconsideration, while its failure counter is incremented ($f_i \leftarrow f_i + 1$). Accumulating failures reduces the strategy's future selection probability, enabling the Playbook to \emph{self-purify} by implicitly filtering out consistently falsified strategies.
    \item \textbf{$E_{uncertain}$ (Inconclusive Evidence)}: Triggered when metric changes are negligible ($|\Delta \mathcal{M}| \le \tau$) or inconsistent, often due to simulator stochasticity or weak attribution. The strategy returns to \textsc{Open} without updating reliability counters, avoiding premature confirmation or rejection.
\end{itemize}

\input{latex/table/state_transition_table}

\subsubsection{Semantic Merging \& Persistence}
\label{ssec:playbook_merge}
% Over long horizons, agents may re-encounter previously addressed issues. To prevent redundancy and enforce historical continuity, we employ a semantic merging mechanism. 
% When a new feedback entry $S_{new}$ is generated, we calculate its similarity to existing strategies $S_{hist} \in \mathcal{K}$:
% \begin{equation}
% \begin{aligned}
% \textsc{Sim}(S_{\text{new}}, S_{\text{hist}})
% &= \alpha \cdot \textsc{Jac}(\textsc{Refs}) \\
% &\quad + \beta \cdot \textsc{Cos}(\mathbf{v}_{\text{new}}, \mathbf{v}_{\text{hist}}).
% \end{aligned}
% \end{equation}
% where $\text{Jac}(Refs)$ is the Jaccard similarity of the Blueprint reference paths (anchoring the bug to the schema), and $\text{Cos}(\cdot)$ is the cosine similarity of SBERT embeddings of the root cause analysis.
% If $Sim > \delta_{thresh}$, the event $E_{merge}$ is triggered. Instead of creating a duplicate, $S_{new}$ updates the content of $S_{hist}$ while \textbf{inheriting} the historical meta-info:
% $u_{new} \leftarrow u_{hist}, s_{new} \leftarrow s_{hist}, f_{new} \leftarrow f_{hist}$.
% This persistence ensures that even if a strategy is reset to \textsc{Open} due to recurrence, the agent retains the ``memory'' of its past reliability, preventing the redundant exploration of historically failure-prone paths.
% This persistence ensures that even if a strategy is reset to \textsc{Open} due to recurrence, the agent retains a quantitative estimate of its historical reliability. Note that the inherited meta-info does not imply correctness; it only encodes accumulated evidence about whether the remediation hypothesis tends to help or hurt. This design enables hypothesis testing over iterations and prevents repeatedly trusting strategies that have been empirically falsified.
Over long horizons, the agent may re-encounter previously diagnosed issues. To avoid redundant entries and preserve historical continuity, we merge new feedback with an existing strategy when they are semantically similar (above a fixed threshold). Instead of creating duplicates, the matched strategy is refreshed with the new diagnosis while inheriting its historical meta-info $(u_i, s_i, f_i)$, so the system retains an evidence-based estimate of reliability across iterations. Importantly, a strategy is treated as a \emph{remedial hypothesis} rather than ground truth: repeated regressions increase its failure count and automatically down-weight its future selection, preventing the agent from repeatedly trusting empirically falsified suggestions.

\subsection{Context Engineering via Knapsack Selection}
\label{sec:context_engineering}

Given the limited context window of LLMs, simply retrieving all historical insights is infeasible. \socia treats prompt construction as a resource allocation problem, ensuring that the agent is presented with the most actionable and \emph{high-utility remedial strategies}---i.e., remediation hypotheses with strong empirical support and high relevance to the current metric failures---to guide the next iteration.

\subsubsection{Evidence-Based Diagnosis}
The foundation of effective context retrieval is accurate grounding. To bridge the numerical results of the inner loop with the symbolic reasoning of the Playbook, the Feedback Agent is constrained to perform \textbf{Evidence-Based Diagnosis}. 
When generating feedback $F_t$, the agent must explicitly bind every identified structural defect to a specific subset of metrics from the \textsc{AvailableMetricKeys} defined in the Blueprint $\mathcal{B}$. 
Formally, a feedback entry is a mapping $f: \text{CodeDefect} \rightarrow \{m \in \mathcal{M} \mid m \text{ is degraded}\}$. 

\subsubsection{Knapsack-Based Context Optimization}
\label{ssec:knapsack}
We model the selection of strategies for the next prompt as a \textbf{0-1 Knapsack Problem}. Let $\mathcal{K}_{cand} \subset \mathcal{K}$ be the set of eligible strategies (status $\in \{\textsc{Open}, \textsc{Queued}\}$). For each strategy $S_i$, let $c_i$ denote its token cost and $v_i$ its estimated value. The objective is to select a subset indicator vector $\mathbf{x} \in \{0, 1\}^{|\mathcal{K}_{cand}|}$ to:

\begin{equation}
    \text{maximize} \sum_{i} v_i x_i \quad \text{s.t.} \quad \sum_{i} c_i x_i \le L_{budget}
\end{equation}

where $L_{budget}$ is the token budget allocated for historical context. The valuation function $v_i$ aggregates multiple utility dimensions:

\begin{equation}
    v_i = w_{user} \cdot w_{sev} \cdot U_{urgency}(t) \cdot \Phi_{reliability}(S_i)
\end{equation}

Here, $w_{user}$ prioritizes strategies tagged as \textit{user-origin} (derived from the HITL interface), while $w_{sev}$ quantifies issue severity. We define $w_{sev}$ according to a discrete scale: \textsc{Blocker} (1.0), \textsc{High} (0.8), \textsc{Medium} (0.6), and \textsc{Low} (0.4), where a \textsc{Blocker} denotes a critical failure preventing simulator execution. 
$U_{urgency}(t)$ is a time-dependent function that increases for strategies languishing in the \textsc{Queued} state, preventing starvation.
Crucially, $\Phi_{reliability}$ estimates the historical effectiveness of strategy $S_i$ using a \textbf{Bayesian posterior mean} over a Beta distribution prior:
\begin{equation}
\begin{aligned}
\Phi_{\text{rel}}(S_i)
&= \mathbb{E}\!\left[\text{Beta}(s_i + 1,\, f_i + 2)\right] \\
&= \frac{s_i + 1}{s_i + f_i + 2}.
\end{aligned}
\end{equation}
where $s_i$ and $f_i$ are the success and failure attributions inherited from the Playbook's meta-info. 
This formulation naturally penalizes strategies with repeated failures (high $f_i$), thereby prioritizing remediation hypotheses that are empirically validated while suppressing consistently falsified or misleading suggestions that may arise from LLM misattribution.

\subsubsection{Strategic Prompt Layout: Countering the ``Lost in the Middle'' Effect}
\label{ssec:lost_in_the_middle}
Selecting high-value strategies is insufficient if the LLM ignores them. Recent findings on the "Lost in the Middle" phenomenon suggest that LLMs attend most strongly to the beginning (Primacy) and end (Recency) of the context window.
We leverage this by restructuring the \socia prompt layout $C_{prompt}$ into three distinct zones:

\begin{enumerate}
    \item \textbf{System Zone (Primacy)}: Contains the agent role definition and rigid output schemas. This establishes the fundamental behavioral constraints.
    \item \textbf{Background Zone (Middle)}: Contains the lengthy $P_{prev}$ (previous code) and $\mathcal{D}_{sim}$ (simulation logs). These serve as reference materials which the model retrieves from but does not need to attend to actively for instruction adherence.
    \item \textbf{Instruction Zone (Recency)}: Crucially, we place the \textbf{Blueprint} $\mathcal{B}$ and the \textbf{Selected Strategies} $\mathcal{S}_{sel}$ at the very end of the prompt, immediately preceding the generation token. 
\end{enumerate}

By positioning the selected remedial strategies $\mathcal{S}_{sel}$ in the Recency Zone, we maximize the probability that the agent conditions on the most relevant \emph{validated remediation hypotheses} at the moment of code synthesis, thereby reducing regressions and preventing repeated execution of previously falsified fixes.

Overall, the Playbook operationalizes long-horizon simulator repair as an evidence-driven hypothesis-testing process: remedial strategies are proposed, validated (or falsified) by metric outcomes, and retained only when repeatedly supported by empirical improvements.

==> latex/table/state_transition_table_verbose.tex <==
\begin{table*}[t]
\centering
\small
\caption{State Transition Logic for Strategy Playbook. Strategies evolve based on selection decisions and metric-driven feedback events.}
\label{tab:state_transition}
\begin{tabular}{@{}llcl@{}}
\toprule
\textbf{Current State} & \textbf{Event} & \textbf{New State} & \textbf{Description} \\ \midrule
(None) & $E_{new}$ & \textsc{Open} & New issue discovered; added to pool. \\
\textsc{Open} & $E_{selected}$ & \textsc{InProgress} & Selected for current prompt context. \\
\textsc{Queued} & $E_{selected}$ & \textsc{InProgress} & Backlog item promoted to context. \\
\textsc{Open} & $not\_selected$ & \textsc{Queued} & Insufficient budget; moved to backlog. \\
\textsc{Queued} & $not\_selected$ & \textsc{Queued} & Remains in backlog. \\ \midrule
\textsc{InProgress} & $E_{resolved}$ & \textsc{Resolved} & Metric improved ($\Delta > \tau$); fix verified. \\
\textsc{InProgress} & $E_{falsified}$ & \textsc{Open} & Metric degraded ($\Delta < -\tau$); failed. \\
\textsc{InProgress} & $E_{uncertain}$ & \textsc{Open} & Signal unclear; returned to pool. \\ \midrule
$\forall \Sigma \in \mathcal{Q}$ & $E_{merge}$ & \textsc{Open} & Recurrence of issue; merged \& reset. \\ \bottomrule
\end{tabular}
\end{table*}
